Designing Reconfigurable Interconnection Network of Heterogeneous Chiplets Using Kalman Filter

Heterogeneous chiplets have been proposed for accelerating high-performance computing tasks. Integrated inside one package, CPU and GPU chiplets can share a common interconnection network that can be implemented through the interposer. However, CPU and GPU applications have very different traffic patterns in general. Without effective management of the network resource, some chiplets can suffer significant performance degradation because the network bandwidth is taken away by communication-intensive applications. Therefore, techniques need to be developed to effectively manage the shared network resources. In a chiplet-based system, resource management needs to not only react in real-time but also be cost-efficient. In this work, we propose a reconfigurable network architecture, leveraging Kalman Filter to make accurate predictions on network resources needed by the applications and then adaptively change the resource allocation. Using our design, the network bandwidth can be fairly allocated to avoid starvation or performance degradation. Our evaluation results show that the proposed reconfigurable interconnection network can dynamically react to the changes in traffic demand of the chiplets and improve the system performance with low cost and design complexity.

==> reference-names.tex <==
1- (modular-R) @INPROCEEDINGS{8416868,
  author={Yin, Jieming and Lin, Zhifeng and Kayiran, Onur and Poremba, Matthew and Shoaib Bin Altaf, Muhammad and Enright Jerger, Natalie and Loh, Gabriel H.},
  booktitle={2018 ACM/IEEE 45th Annual International Symposium on Computer Architecture (ISCA)}, 
  title={Modular Routing Design for Chiplet-Based Systems}, 
  year={2018},
  volume={},
  number={},
  pages={726-738},
  keywords={Routing;System recovery;Graphics processing units;Silicon;Computer architecture;Topology;Government;chiplet;deadlock-avoidance;routing},
  doi={10.1109/ISCA.2018.00066}}

